Measurements of the $\tau$ Mass and Mass Difference of the $\tau^{+}$ and $\tau^{-}$} at BaBar

We present the result from a precision measurement of the mass of the $\tau$ lepton, $M_\tau$, based on $423 fb^{-1}$ of data recorded at the $\Upsilon(4S)$ resonance with the BaBar detector. Using a pseudomass endpoint method, we determine the mass to be $1776.68 \pm 0.12 (stat) \pm 0.41 (syst) MeV$. We also measure the mass difference between the $\tau^+$ and $\tau^-$, and obtain $(M_{\tau^{+}}-M_{\tau^{-}})/M^\tau_{AVG} = (-3.4 \pm 1.3 (stat) \pm 0.3 (syst)) \times 10^{-4}$, where $M^\tau_{AVG}$ is the average value of $M_{\tau^+}$ and $M_{\tau^-}$.

==> abstract.tex <==
We present the result from a precision measurement of the mass of the $\tau$ lepton, $M_\tau$, based on $423~fb^{-1}$ of data recorded at the $\Upsilon(4S)$ resonance with the BaBar detector.  Using a pseudomass endpoint method, we determine the mass to be $1776.68 \pm 0.12 (stat) \pm 0.41 (syst)~MeV$.  We also measure the mass difference between the $\tau^+$ and $\tau^-$ , and obtain $(M_{\tau^{+}}-M_{\tau^{-}})/M^\tau_{AVG} = (-3.4 \pm 1.3 (stat) \pm 0.3 (syst)) \times 10^{-4}$, where $M^\tau_{AVG}$ is the average value of $M_{\tau^+}$ and $M_{\tau^-}$.

==> acknowledgements.tex <==
We are grateful for the 
extraordinary contributions of our \pep2\ colleagues in
achieving the excellent luminosity and machine conditions
that have made this work possible.
The success of this project also relies critically on the 
expertise and dedication of the computing organizations that 
support \babar.
The collaborating institutions wish to thank 
SLAC for its support and the kind hospitality extended to them. 
This work is supported by the
US Department of Energy
and National Science Foundation, the
Natural Sciences and Engineering Research Council (Canada),
the Commissariat \`a l'Energie Atomique and
Institut National de Physique Nucl\'eaire et de Physique des Particules
(France), the
Bundesministerium f\"ur Bildung und Forschung and
Deutsche Forschungsgemeinschaft
(Germany), the
Istituto Nazionale di Fisica Nucleare (Italy),
the Foundation for Fundamental Research on Matter (The Netherlands),
the Research Council of Norway, the
Ministry of Education and Science of the Russian Federation, 
Ministerio de Educaci\'on y Ciencia (Spain), and the
Science and Technology Facilities Council (United Kingdom).
Individuals have received support from 
the Marie-Curie IEF program (European Union) and
the A. P. Sloan Foundation.


